Inversion Ring in Chromonic Twisted Hedgehogs: Theory and Experiment

Twisted hedgehogs are defects in spherical cavities with homeotropic anchoring for the nematic director that arise when twist distortions are sufficiently less energetic than splay (and bend) distortions. They bear a characteristic inversion ring, where the director texture changes the sense it spirals about the center of the cavity. This paper applies a quartic twist theory recently proposed to describe the elasticity of chromonics to explain a series of inversion rings observed in aqueous solutions of SSY at two different concentrations. The theory features a phenomenological length a, whose measure is extracted from the data and shown to be fairly independent of the cavity radius, as expected for a material constant.

==> caption/CHANGELOG <==
Changes made in the caption package bundle
==========================================

Please note that this document does not reflect bugfix-releases (which are marked with a letter after the version number, for example v3.4m), and that the dates given are the dates of the release w/o bugfixes.

If you are interested in a complete changelog -- including bugfixes -- process the dtx files with \RecordChanges and \PrintChanges.


caption package
---------------

v1.0 (1994/10/27)
- 1st published version

v1.1 (1994/11/03)
- New option `centerlast'

v1.2 (1994/11/28)
- Support of the `float' package added

v1.3 (1995/01/09)
- Support of \captionlabelfont in subcaptions added

v1.4 (1995/01/30)
- New option `nooneline'

v2.0 (caption2, 1995/10/09)
- New experimental version with many new commands and features
- Support of the `longtable' package added

v2.1 (caption2, 2002/02/26)
- Adapted to version 2.1 of the subfigure package
- New options for interaction with other packages (float,...)
- New command \normalcaptionparams
- New commands \captionof and \captionof*
- New ifs \ifcaptionlabel and \ifignoreLTcapwidth
- \realcaptionwidth renamed to \captionlinewidth

v2.2 (caption2, 2007/04/06)
- Internal change: Uses the caption3 kernel now

v3.0 (2003/12/20)
- Completely rewritten in cooperation with Frank Mittelbach and Steven Cochran

v3.1 (2007/09/01)
- Improved compatibility to supported document classes and packages, but decreased compatibility to non-supported document classes and packages
- Support of the AMS & SMF document classes added
- Support of the `beamer' document class added
- Support of the `KOMA-Script' document classes added
- Support of the `floatflt' package added
- Support of the `fltpage' package added
- Support of the `picinpar' package added
- Support of the `picins' package added
- Support of the `threeparttable' package added
- Support of the `wrapfig' package added
- Support of the `xtab' package added
- Check against incompatible `ftcap' package added
- Check against incompatible `nonfloat' package added
- Check against incompatible `topcapt' package added
- Does not process global options anymore to avoid conflicts with document class options
- New option compatibility=
- New options font+=, labelfont+= & textfont+=
- New options hypcap= & hypcapspace=
- New options list= and listformat=
- New option options=
- New options figurewithin= and tablewithin=
- Starred variant of option margin*= added
- Starred variant of option style*= added
- Starred variant of option type*= added
- Font options `normal', `normalcolor', `color', `normalfont' & `stretch' added
- Default position changed from `bottom' to `auto'
- New command \DeclareFloatingEnvironment resp. \DeclareCaptionType
- New command \DeclareCaptionListFormat
- New command \captionlistentry
- Starred variant of \clearcaptionsetup added
- Optional argument added to \clearcaptionsetup
- Starred variant of \ContinuedFloat added
- \captionsetup{...} inside longtables added
- \captionsetup[singleline]{...} added
- A \label before \caption will result in warning "\label before \caption ignored"
- The counters lofdepth & lotdepth are supported now
- Label formats have three arguments now
- Optional argument added to \DeclareCaptionFormat; "format=plain" removed from single-line options of default format
- Caption label format `brace' added

v3.2 (2011/07/30)
- Support of `beamer' document class improved
- Support of `magyar' babel option added
- Support of `sansmath' package added
- Support of `titletoc' package added to \DeclareCaptionType & \DeclareCaptionSubType
- Support of `tocbasic' package added to \DeclareCaptionType
- New options calcmargin=, calcmargin*=, calcwidth=, and calcwidth*=
- New option listtype= added
- New option parboxrestore=partial/full
- New options within= & without
- Option slc= as abbreviation of singlelinecheck= added
- Pre-defined text format `empty' added
- New command \captionbox
- New command \phantomcaption
- New command \setcaptiontype as replacement for \captionsetup{type=...}
- New command \setcaptionsubtype as replacement for \captionsetup{subtype}
- "Hyperref support is turned off because hyperref has stopped early" is not a warning anymore but an information instead

v3.3 (2013/01/06)
- Revised handling of continued floats and sub-captions
- New option box= and appropriate command \DeclareCaptionBox
- New option list-entry= (see also endfloat package documentation)
- Support of multiple optional arguments added to \captionsetup (see bicaption package documentation)
- Adapted to the elsarticle document class
- Adapted to the current version of memhfixc package, provided by the memoir document class
- Fixed compatibility problem with breqn and nag packages
- Corrects incorrect load order hyperref-float now (needs hyperref v6.82q or newer)
- New switch \ifsinglelinecaption for usage inside own commands added

v3.4 (2019/09/11)
- Label format `autodot' added (for usage within documents using KOMA-Script document class)
- Label format `unnumbered' added
- \ContinuedFloat renamed to \continuedfloat (since this is not a preamble command)
- \caption will always be re-defined now, unless `compatibility' is set to `true' (or an incompatible package is loaded)

v3.5 (2020/08/30)
- If a document class defines \caption@documentclass, an adaption to the caption package will be loaded as caption-<documentclass>.sto
- New commands \SetCaptionDefault, \AtCaptionPackage, and \AfterCaptionPackage for usage in document classes or document class adaptions
- Document class support re-written (using the new commands above)
- New commands \caption@switchdefault and \caption@restoredefault for usage in babel language packages
- Babel language support re-written (using the new commands above); furthermore it's independent on the load order now
- Support for the babel language option `latvian' added
- New command \DeclareCaptionSinglelinecheck
- New commands \ForEachCaptionType and \ForEachCaptionSubType
- Options "figure*" resp. "table*" will be applied additionally in "figure*" resp. "table*" environments (twocolumn mode only)
- Option and font option "hypersetup" added which expands to \hypersetup (if defined) resp. nothing (otherwise)

v3.6 (2022/02/20)
- Fallback to versions "v1", "v3.0", "v3.1", "v3.2", "v3.3", "v3.4", and "v3.5" added
- The caption-subcaption counter handling is now independent on the "position=" setting
- Option "compatibility=true" dropped in favor of "\usepackage{caption}[=v1]"
- Option "parboxrestore=partial/full" removed (was obsolete since v3.5)
- \captionsetup{margin={...,}} sets only the left margin, \captionsetup{margin={,...}} only the right one
- The font option "stretch" does not require the setspace package anymore
- New command \nextfloat to influence the (new) counter handling
- New command \DeclareCaptionPosition to declare custom postion settings
- New command \AtCaptionSingleLineCheck to add re-definitions to the single-line-check
- New command \captiontext to typeset a caption without counter increment and without list entry
- Optional argument added to \setcaptiontype (which specifies options to be applied additionally)
- New environments `captiongroup' and `captionblock'
- Adapted to the `tablefootnote' package


bicaption package
-----------------

v0.9 (2010/09/19)
- 1st published version (see also http://www.mrunix.de/forums/showthread.php?t=68312)

v1.0 (2011/09/03)
- Support for list entries added

v1.1 (2012/12/26)
- \captionmainlanguage and \selectcaptionlanguage added

v1.2 (2016/03/27)
- \DeclareLangDependantCaptionOption added

v1.3 (2020/10/25)
- Option "bi-separator" and command \DeclareBiCaptionSeparator added

v1.4 (2020/12/25)
- Support of all available caption fallback versions since "v3.2" added

v1.5 (2021/01/04)
- Support of the listings package added

v1.6 (2023/02/19)
- Command \bicaptionsetup added


ltcaption package
-----------------

v1.0 (2007/04/15)
- 1st version

v1.1 (2007/09/01)
- Adapted to the NTG document classes (Support of \CaptionLabelFont & \CaptionTextFont added)
- Adapted to the `floatrow' package by Olga Lapko
- New macro \LTcaptype
- New environment longtable*

v1.2 (2008/03/28)
- New skip \LTcapskip

v1.3 (2011/09/12)
- New macro \CaptionLabelSeparator

v1.4 (2013/06/01)
- Adapted to the memoir document class (v3.7b)


subcaption package
------------------

v1.0 (2008/03/16)
- 1st published version

v1.1 (2011/08/17)
- New caption option subrefformat=
- New command \phantomsubcaption

v1.2 (2018/05/13)
- Values `B' and `T' for the optional argument <outer-pos> added to the environments `subfigure' and `subtable'

v1.3 (2019/08/31)
- New command \subfloat for easy transition from the `subfig' package

v1.4 (2020/12/25)
- Support of all available caption fallback versions since "v3.1" added

v1.5 (2022/01/07)
- New environments subcaptiongroup and subcaptionblock
- New command \subcaptionlistentry to make an entry into the list of figures resp. tables
- New command \subcaptiontext to typeset a sub-caption without counter increment and list entry
- Default value of the optional argument <outer-pos> changed from `c' to either `b' or `t'

v1.6 (2023/02/19)
- New command \subcaptionsetup to set options specifically for sub-captions
- Counter ownership revised


==> caption/README <==
==========================================================================

The `caption' package bundle
Release 2023-09-08
Copyright (C) 1994-2023 Axel Sommerfeldt (axel.sommerfeldt@f-m.fm)

License: LPPL = LaTeX Project Public Licence
Maintenance Status: maintained (by Axel Sommerfeldt)

Home page:
  https://gitlab.com/axelsommerfeldt/caption

If you need help for installation please visit:
  https://texfaq.org/FAQ-inst-miktexstar
  https://texfaq.org/FAQ-installthings
  https://texfaq.org/FAQ-privinst

If you need help using these packages please visit:
  https://latex.org/forum/
  https://topanswers.xyz/tex
  https://tex.stackexchange.com/
  https://golatex.de/               (German)
  https://texwelt.de/               (German)

If you think you may have found a bug in these packages,
or want to report a suggestion for improvement, please either visit
  https://gitlab.com/axelsommerfeldt/caption/issues
or send an e-mail to
  axel.sommerfeldt@f-m.fm

--------------------------------------------------------------------------

The `caption' package v3.6 offers customization of captions of floating
environments such `figure' and `table' and cooperates with the packages

  float, floatflt, fltpage, hyperref, hypcap, listings, longtable,
  picinpar, picins, rotating, sidecap, subfigure, supertabular,
  threeparttable, wrapfig, and xtab.

Furthermore the `floatrow', the `subcaption', and the `subfig' package
supports the `caption' package and uses its \captionsetup interface.

User Manual: caption.pdf (English, currently in review)

Outdated user manuals in Russian and German could be downloaded from
https://gitlab.com/axelsommerfeldt/caption/-/tree/master/doc/outdated

--------------------------------------------------------------------------

The `bicaption' package v1.6 supports typesetting of bilingual captions.

User Manual: bicaption.pdf (English)

--------------------------------------------------------------------------

The `ltcaption' package v1.4 fixes caption problems with
other-than-center aligned longtables. (solving LaTeX PR `tools/3387')

A bonus feature is the addition of the environment longtable* which does
not increment the table counter.

This package will be loaded automatically by the `caption' package,
but can be used without the caption package, too.

User Manual: ltcaption.pdf (English)

--------------------------------------------------------------------------

The `subcaption' package v1.6 supports typesetting of sub-captions
(by using the the sub-caption feature of the `caption' package).

User Manual: subcaption.pdf (English)

--------------------------------------------------------------------------

Note: The `newfloat' package was removed from this package bundle and was
uploaded to CTAN as stand-alone package.

Note: The `totalcount' package was removed from this package bundle and
was uploaded to CTAN as stand-alone package.

==========================================================================
(The pictures cat.eps & elephant.eps were taken with permission from the
 LaTeX Companion examples.)

